LLM-enhanced Scene Graph Learning for Household Rearrangement

The household rearrangement task involves spotting misplaced objects in a scene and accommodate them with proper places. It depends both on common-sense knowledge on the objective side and human user preference on the subjective side. In achieving such task, we propose to mine object functionality with user preference alignment directly from the scene itself, without relying on human intervention. To do so, we work with scene graph representation and propose LLM-enhanced scene graph learning which transforms the input scene graph into an affordance-enhanced graph (AEG) with information-enhanced nodes and newly discovered edges (relations). In AEG, the nodes corresponding to the receptacle objects are augmented with context-induced affordance which encodes what kind of carriable objects can be placed on it. New edges are discovered with newly discovered non-local relations. With AEG, we perform task planning for scene rearrangement by detecting misplaced carriables and determining a proper placement for each of them. We test our method by implementing a tiding robot in simulator and perform evaluation on a new benchmark we build. Extensive evaluations demonstrate that our method achieves state-of-the-art performance on misplacement detection and the following rearrangement planning.

==> cover_letter.tex <==
Dear Reviewers,

In this letter, we explain how we addressed the concerns listed in the summary review. The corresponding changes in the revision are highlighted in blue color.

1.	Incorporate all mentioned and promised details and clarifications in the rebuttal.

1）	We present another application of our affordance-enhanced graph for the human activity heat map generation task in Section F of the supplementary materials.

2）	A detailed description of the initial scene graph construction and scene graph enhancement, as well as the pseudo-code of their pipelines, have been added in Section B.1 and B.3 of the supplementary materials.

3）	A new ablation study on key frame selection has been added in Section E.1 of the supplementary materials.


4）	An ablation study on the value of K is included in Section E.2 of the supplementary materials.

5）	We have included ablation studies on scoring methods and provided more detailed explanations of the prompting choices in Section C and Section E.3 of the supplementary materials.

6）	A clearer explanation of the two datasets and their differences is provided in Section 4.1 (Lines 603-622), with further details available in Section C.1 of the supplementary materials. Additionally, a brief introduction to the NDCG metric and HouseKeep [Kant et al. 2022] is included in Section 4.1 (Lines 649-659) and Section 4.2 (Lines 678-683).

6）	A clearer explanation of the the classification of rearrangement type has been added in Section A of the supplementary materials. Additionally, the generalization of the experimental setting is discussed in Section A and Section F of the supplementary materials

2.	Further discussion and clarifications surrounding how to exactly identify and conform with specific "user preference.

>> We revised our paper to include additional explanations clarifying how our method extracts specific user preferences by leveraging scene contexts. These clarifications can be found in Lines 101-103, 108-112, 124-128, 333-335, and 372-375.

3.	Incorporate changes and additional discussions that help selling this paper to a more general audience.

>> In addition to rephrasing certain expressions in the paper to enhance clarity for the audience, we have included additional cases in Section F of the supplementary materials to demonstrate how our method can be applied to other tasks. 


Thank you, 
The authors


